S$^{3}$: Increasing GPU Utilization during Generative Inference for Higher Throughput

Generating texts with a large language model (LLM) consumes massive amounts of memory. Apart from the already-large model parameters, the key/value (KV) cache that holds information about previous tokens in a sequence can grow to be even larger than the model itself. This problem is exacerbated in one of the current LLM serving frameworks which reserves the maximum sequence length of memory for the KV cache to guarantee generating a complete sequence as they do not know the output sequence length. This restricts us to use a smaller batch size leading to lower GPU utilization and above all, lower throughput. We argue that designing a system with a priori knowledge of the output sequence can mitigate this problem. To this end, we propose S$^{3}$, which predicts the output sequence length, schedules generation queries based on the prediction to increase device resource utilization and throughput, and handle mispredictions. Our proposed method achieves 6.49$\times$ throughput over those systems that assume the worst case for the output sequence length.

==> 4-analysis.tex <==
\section{Analysis: misprediction penalty of \name}

\name\ is a genAI serving system that schedules requests with sequence length predictions. We analyze the tow penalties: 1) eviction penalty and 2) underutilization penalty, and show how much benefit we achieve from our design. 

\subsection{Eviction Penalty}
% \name\ has to move sequences from device (GPU) to the host DRAM when the prediction results is shorter than the actual sequence length.
The first penalty of a misprediction is the eviction penalty where \name\ has to transfer the states of the mispredicted sequence to the host DRAM and release the memory held by the sequence. This includes the KV cache of the sequence along with its current hidden state. The size of the KV cache is orders of magnitude larger than that of the hidden state thus we disregard the hidden state's size in the below analysis.

Let $p$ be the probability that the predicted sequence length is shorter than the actual sequence length. The eviction penalty is observed only when $p > 0$ (there exist some predictions that are shorter than the actual length). In such a case, the cost of evicting a sequence from the GPU HBM and loading it back to the HBM is $2\frac{S_P(x_s)}{BW_{HD}}$ with $x_s \in PS$ and $PS = \{x | S_P(x) < S_A(x)\}$ where $S_P(x)$ represents the key and value caches' size generated from the predicted length, $S_A(x)$ the size generated from the actual length, and $BW_{H2D}$ the memory bandwidth of the connection between the CPU (i.e., host) and the GPU (i.e., device).

We also analyze the cost of rearranging the remaining sequences in the GPU HBM. This must be done after evicting a sequence from the HBM such that there are no holes in the matrix representation of our sequences. For example, assume that a $m\times n$ matrix $M$ represents a batch of sequences where each row corresponds to each sequence and each column corresponds to each element in the embedding vector. Evicting the row $i$ from the matrix will cause memory fragmentation and will leave a hole in the middle of the vector. Therefore, we shift upwards the rows below the row $i$ so that the rows are stored contiguously in the HBM. We read on average $\frac{m}{2}$ rows and write them back assuming that the positions of the rows to be evicted follow a uniform distribution. 

Combining the eviction and the rearrangement, we can represent the total eviction penalty of the evicting sequence $x_i$ from the HBM with $n$ sequences as

\[
     2(\frac{S_P(x_i)}{BW_{H2D}} + \frac{\sum_{i+1}^{n}{S_P(x_j)}}{BW_{HBM}})
\]

 and the total eviction penalty in a request pool of N sequences is
 
\[
     2pN(\frac{S_P(x)}{BW_{H2D}} + \frac{\sum_{0}^{n}{S_P(x_j)}}{2BW_{HBM}})
\]

if the position of the evicted row follows a uniform distribution. 

The above equation gives as several insights on the eviction penalty. In the algorithm side, the eviction penalty does not exist as long as the predictor does not make any short predictions. That is, the predictor can make long mispredictions but we will not see any eviction penalties. In the systems side, we can see that the eviction penalty is dependent only on the memory bandwidths. Thus, we can lower the eviction penalty by using memory and interconnects with higher throughput and lower latency.
%\color{blue}{How serious is the problem?}

\subsection{Underutilization Penalty}
% When a prediction result si longer than the actual sequence length.

The second penalty of a misprediction is the GPU resource underutilization due to smaller batch size. This penalty is observed when the sequences in a batch are allocated larger memory than necessary. We analyze the batch size difference between a system with a predictor and the ideal system with an oracle and show the extent of GPU resource underutilization.

We start off by calculating the average predicted sequence length in a request pool to figure out the average number of sequences (i.e., batch size) in a GPU. The average KV cache size in the system with the predictor will be $\frac{\sum^NS_P(x)}{N}$ . Similarly, the average KV cache size calculated from the oracle will be $\frac{\sum^NS_A(x)}{N}$. Assuming that each the predicted length of each sequence is equal to the averaged length, we can achieve the average batch size by dividing GPU HBM capacity by the average KV cache sizes. 

We calculate the batch size difference, hence the underutilization ratio as
\[
    \frac{\sum^NS_A(x)}{\sum^NS_P(x)}
\]
by dividing the batch size in the system with the oracle from that in the system with the predictor. We can infer two takeaways from the equation. First, FasterTransformer suffers from massive underutilization as it allocates the maximum sequence length to each KV cache which can be multiples of the actual sequence length. Second, the underutilization might not be significant even if the predictor makes longer prediction as long as the aggregate of the predictions is similar to the aggregate of the actual length. Furthermore, the system with the predictor can achieve higher utilization if the predictor always makes shorter predictions but this benefit will soon be canceled out by the high eviction penalty.


% with $x_l\in PL$ and $PL= \{x|S_P(x) > S_A(x)\}$
% The second penalty of a misprediction is the underutilization of GPU resources due to smaller batch size. The penalty is observed when the sum predicted length is longer than the sum of actual lengths. \name\ allocates more memory to each sequence than necessary and fills the HBM with fewer sequences compared to allocating the exact size of memory to the sequences. GPU now inferences fewer sequences at a time, resulting in longer latency per sequence and lower thorughput overall. We analyze the extent of underutilization in such cases compared to the ideal case with an oracle. 

%This penalty is observed when $\sum L(x_s) + \sum L(x_l) > \sum A(X)$ where $x_s \in PS$ and $x_l \in PL$ with $PL = \{x | L(X) > A(X)\}$ in a certain batch. That is, \name\ will underutilize the GPU resources if the aggregate predicted length of sequences currently loaded in the HBM is larger than the aggregate of the actual lengths. This would mean that \name\ is allocating more memory than necessary to the loaded sequences and which blocks other sequences to be loaded even with enough free memory to accommodate them.

% We formulate the degree of underutilization in terms of the batch size at a certain time period. We batch sequences such that we maximize the HBM usage. Therefore, the number of sequences in a batch is the inverse of the HBM capacity divided by the average length of sequences in the batch. The batch size of predicted 


% \subsection{Extension to Larger Models}
% \begin{enumerate}
%     \item In case of model parallel inference
%     \item In case of tensor parallel inference
% \end{enumerate}
